Understanding and Detecting Annotation-Induced Faults of Static Analyzers

Static analyzers can reason about the properties and behaviors of programs and detect various issues without executing them. Hence, they should extract the necessary information to understand the analyzed program well. Annotation has been a widely used feature for different purposes in Java since the introduction of Java 5. Annotations can change program structures and convey semantics information without awareness of static analyzers, consequently leading to imprecise analysis results. This paper presents the first comprehensive study of annotation-induced faults (AIF) by analyzing 246 issues in six open-source and popular static analyzers (i.e., PMD, SpotBugs, CheckStyle, Infer, SonarQube, and Soot). We analyzed the issues' root causes, symptoms, and fix strategies and derived ten findings and some practical guidelines for detecting and repairing annotation-induced faults. Moreover, we developed an automated testing framework called AnnaTester based on three metamorphic relations originating from the findings. AnnaTester generated new tests based on the official test suites of static analyzers and unveiled 43 new faults, 20 of which have been fixed. The results confirm the value of our study and its findings.

==> tab-BugProneAnnotations.tex <==
\begin{table}[!tbp]
\caption{Top 10 AIF Prone Annotations}
\label{tab:aifannotation}
\centering
% \resizebox{\linewidth}{!} 
% {
\small
\begin{tabular*}{0.5\linewidth}{@{\extracolsep{\fill} }llr}
\toprule
Rank & Annotation Name & \#Issue \\
\midrule
1 & @Nullable & 26 \\
2 & @NonNull & 18 \\
3 & @SuppressWarnings & 12 \\
4 & @Inject & 8 \\
5 & @Test & 8 \\
6 & @Autowired & 6 \\
7 & @Value & 6 \\
8 & @Data & 6 \\
9 & @CheckForNull & 5 \\
10 & @VisiableForTesting & 4 \\
\bottomrule
\end{tabular*}
% }
\end{table}

% \begin{table}[!tbp]
% \caption{Top 10 AIF Prone Annotations}
% \label{tab:aifannotation}
% \centering
% % \resizebox{\linewidth}{!} 
% % {
% \small
% \begin{tabular*}{\linewidth}{@{\extracolsep{\fill} }lrrrrrrrrrr}
% \toprule
% Rank & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\
% \midrule
% Annotation Name & & @Nullable & @NonNull & @SuppressWarnings & @Inject & &&&
% \bottomrule
% \end{tabular*}
% % }
% \end{table}

==> tab-Experiment.tex <==
% \begin{table}[!tbp]
% \caption{Overall execution time}
% \label{tab:exectime}
% \centering
% % \resizebox{\linewidth}{!} 
% % {
% \begin{tabular*}{\linewidth}{@{\extracolsep{\fill} }lrrrr}
% \toprule
% Static analyzer & SIC & ASC & EAC & Sum \\
% \midrule
% \pmd & & &  \\
% \cstyle & & &  \\
% \sonar & & & \\
% \sbugs & & & \\
% \infer & & & \\
% \bottomrule
% \end{tabular*}
% % }
% \end{table}

\begin{table}[!tb]
\caption{Effectiveness of \sys{}}
\label{tab:experimentresults}
\centering
% \resizebox{\linewidth}{!} 
% {
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill} }lrrrr}
\toprule
Checker & ISC & ASC & EAC & Overall \\
\midrule
Number of found bugs & 21 & 6 & 6 & \faultcnt{} \\
Number of fixed bugs & 7 & 4 & 4 & \fixedfaultcnt{} \\
Number of FPs & 9 & 0 & 0 & 9 \\
Total Running Time (hour) & 62 & 16 & 121 & 199 \\
\bottomrule
\end{tabular*}
% }
\end{table}

==> tab-FixStrategyDistribution.tex <==
\begin{table*}[!htbp]
\caption{Fix strategy distribution}
\label{tab:fixdistribution}
\centering
% \resizebox{\linewidth}{!} 
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\toprule
\textbf{Static analyzer} & FAF & FTM & CMA & FGI & SIA & FVC & FAN & RRC & Others \\
\midrule
\pmd{} & & & & & & & & & \\
\cstyle{} & & & & & & & & & \\
\sonar{} & & & & & & & & & \\
\sbugs{} & & & & & & & & & \\
\infer{} & & & & & & & & & \\
\hline
\textbf{Sum} & & & & & & & & & \\
\bottomrule
\end{tabular}
\end{table*}

==> tab-FixedIssues.tex <==
\begin{table}[!tb]
\caption{\zhe{Distribution of Fix Strategy among Fixed Issues}}
\label{tab:fixedissues}
\centering
% \resizebox{\linewidth}{!} 
% {
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill} }lrrrrrrrr}
\toprule
Fix Strategy & FAF & FAN & FIT & FGI & FVC & RRC & Others & Overall \\
\midrule
Number & 15 & 2 & 0 & 3 & 0 & 1 & 1 & \fixedfaultcnt{} \\
\bottomrule
\end{tabular*}
% }
\end{table}

==> tab-IssueStatus.tex <==
% \begin{table}[htbp]
% \caption{The status of submitted issues}
% \label{tab:issuestatus}
% \centering
% \resizebox{\linewidth}{!} 
% {
% \begin{tabular}{|c|c|}
% \toprule
% Issue status & Number \\
% \midrule
% Fixed & \fixedbugcnt{} \\
% Confirmed & 1 \\
% Pending & xx  \\
% Won't fix & 2 \\
% \hline
% Total & \bugcnt{} \\
% \bottomrule
% \end{tabular}
% }
% \end{table}

\begin{table}[htbp]
\caption{The status of submitted issues}
\label{tab:issuestatus}
\centering
% \resizebox{\linewidth}{!} 
% {
\begin{tabular*}{0.7\linewidth}{@{\extracolsep{\fill} }cc}
\toprule
Issue status & Number \\
\midrule
Fixed & \fixedbugcnt{} \\
Confirmed & 1 \\
Pending & xx  \\
Won't fix & 2 \\
\bottomrule
\end{tabular*}
% }
\end{table}
